Universes for category theory

The Grothendieck universe axiom asserts that every set is a member of some set-theoretic universe U that is itself a set. One can then work with entities like the category of all U-sets or even the category of all locally U-small categories, where U is an "arbitrary but fixed" universe, all without worrying about which set-theoretic operations one may legitimately apply to these entities. Unfortunately, as soon as one allows the possibility of changing U, one also has to face the fact that universal constructions such as limits or adjoints or Kan extensions could, in principle, depend on the parameter U. We will prove this is not the case for adjoints of accessible functors between locally presentable categories (and hence, limits and Kan extensions), making explicit the idea that "bounded" constructions do not depend on the choice of U.

==> Content-04.tex <==
% !TEX root = UniversesForCT.tex
\section{An application in homotopy theory}

The motivating question behind this paper was the following:
\begin{quote}
Let $\mathbb{B}$ be a $\mbfU$-small category with colimits for $\kappa$-small diagrams. Given a combinatorial model structure on $\mathcal{M} = \Ind[\kappa][\mbfU]{\mathbb{B}}$, does it extend to a combinatorial model structure on $\succof{\mathcal{M}} = \Ind[\kappa][\mbfUplus]{\mathbb{B}}$?
\end{quote}
More precisely, if $\mathcal{I}$ is a $\mbfU$-set of generating cofibrations and $\mathcal{J}$ is a $\mbfU$-set of generating trivial cofibrations in $\mathcal{M}$, is there a model structure on $\succof{\mathcal{M}}$ that is cofibrantly generated by $\mathcal{I}$ and $\mathcal{J}$? 

\begin{lem}
\needspace{2.5\baselineskip}
With notation as above:
\begin{enumerate}[(i)]
\item The inclusion $\mathcal{M} \embedinto \succof{\mathcal{M}}$ preserves the functorial factorisations constructed by Quillen's small object argument,\footnote{See \eg Lemma 3 in \citep[\Chap II, \Sect 3]{Quillen:1967}.}

\item Every $\mathcal{I}$-injective morphism in $\succof{\mathcal{M}}$ is also a $\mathcal{J}$-injective morphism.

\item Every $\mathcal{J}$-cofibration in $\succof{\mathcal{M}}$ is also an $\mathcal{I}$-cofibration.
\end{enumerate}
Now, define $\succof{\mathcal{W}}$ to be the collection of all morphisms in $\succof{\mathcal{M}}$ of the form $q \circ j$ for a $\mathcal{J}$-cofibration $j$ and a $\mathcal{I}$-injective morphism $q$. Then:
\begin{enumerate}[resume*]
\item Any $\mathcal{I}$-cofibration in $\succof{\mathcal{M}}$ that is also in $\succof{\mathcal{W}}$ is a (retract of a) $\mathcal{J}$-cofibration.

\item Any $\mathcal{J}$-injective morphism in $\succof{\mathcal{M}}$ that is also in $\succof{\mathcal{W}}$ is a (retract of a) $\mathcal{I}$-injective morphism.
\end{enumerate}
\end{lem}
\begin{proof}
Use \autoref{prop:accessible.extensions.preserve.colimits} and \autoref{thm:accessible.extension.properties}.
\end{proof}

\begin{thm}
With other notation as above, let $\succof{\mathcal{C}}$ be the collection of all $\mathcal{I}$-injective morphisms in $\succof{\mathcal{M}}$, and let $\succof{\mathcal{F}}$ be the collection of all $\mathcal{J}$-injective morphisms in $\succof{\mathcal{M}}$. [...]
\end{thm}

==> Prelude0.tex <==
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}

\ifdefined\ifdraftdoc

\else
  \usepackage{ifdraft}
  \makeatletter
  \let\ifdraftdoc\if@draft
  \makeatother
\fi

\usepackage{needspace}

\usepackage{multirow}
\usepackage[leqno]{amsmath}
\allowdisplaybreaks[4]
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}

\renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\openqedsymbol}{$\square$}
\newcommand{\exercisesymbol}{$\lozenge$}
\newcommand{\obvioussymbol}{$\blacklozenge$}
\newcommand{\openproof}{\renewcommand{\qedsymbol}{\openqedsymbol}}
\newcommand{\exerproof}{\renewcommand{\qedsymbol}{\exercisesymbol}}
\newcommand{\obviousproof}{\renewcommand{\qedsymbol}{\obvioussymbol}}

\usepackage{mathrsfs}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\usepackage{stmaryrd}

\usepackage{mathtools}

\usepackage[british]{babel}

\usepackage[autostyle]{csquotes}
\usepackage{hyphenat}

\usepackage{etoolbox}
\usepackage{xstring}

\usepackage[shortlabels]{enumitem}

\usepackage[dvipsnames,hyperref]{xcolor}

\usepackage{tikz}
\usepackage{tikz-cd}

\usetikzlibrary{arrows, shapes.geometric}
\usetikzlibrary{decorations.pathmorphing}
\tikzset{baseline=(current bounding box.center)}

\let\LiningNumbers\relax

\linespread{1.1}

\DeclareTextFontCommand{\textrmup}{\rmfamily\mdseries\upshape}
\DeclareTextFontCommand{\textbfup}{\rmfamily\bfseries\upshape}
\DeclareTextFontCommand{\textttup}{\ttfamily\mdseries\upshape}
\DeclareTextFontCommand{\textsfup}{\sffamily\mdseries\upshape}

\setlist[enumerate]{font=\upshape}

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{mb}{it}{
   <-> s * [1.150] pzcmi7t
}{}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{mb}{it}

\DeclareMathSymbol{\epsilon}{\mathord}{letters}{"22}
\DeclareMathSymbol{\phi}{\mathord}{letters}{"27}
\DeclareMathSymbol{\varepsilon}{\mathord}{letters}{"0F}
\DeclareMathSymbol{\varphi}{\mathord}{letters}{"1E}

\usepackage{microtype}

\makeatletter
\newcommand*{\noprelistbreak}{\@nobreaktrue\nopagebreak}
\makeatother

\usepackage{xspace}

\newcommand{\hairspace}{\ifmmode\mskip1mu\else\kern0.08em\fi}
\newcommand{\mmhfill}{\hskip \textwidth minus \textwidth}

\makeatletter
\def\abbrdot{\@ifnextchar.{}{.\@\xspace}}
\makeatother
\newcommand{\etc}{etc\abbrdot}
\newcommand{\eg}{e.g\abbrdot}
\newcommand{\ie}{i.e\abbrdot}
\newcommand{\resp}{resp\abbrdot}
\newcommand{\confer}{cf\abbrdot}
\newcommand{\loccit}{loc.\@ cit\abbrdot}
\newcommand{\opcit}{op.\@ cit\abbrdot}

\newcommand{\Chap}{Ch.\@~}
\newcommand{\Appx}{App.\@~}
\newcommand{\Sect}{\S\hairspace}
\newcommand{\Sects}{\S\S\hairspace}
%\newcommand{\textnumero}{N\textsuperscript{\underline{o}}\xspace}
\newcommand{\Numero}{N\textsuperscript{\underline{o}}~}

\newcommand{\strong}[1]{\textbfup{#1}}

\renewcommand{\implies}{\ifmmode\Longrightarrow\else$\Rightarrow$\expandafter\xspace\fi}
\renewcommand{\iff}{\ifmmode\Longleftrightarrow\else$\Leftrightarrow$\expandafter\xspace\fi}

\makeatletter
\let\internal@prime\prime
\renewcommand{\prime}{\ifmmode\internal@prime\else$\sp{\internal@prime}$\expandafter\xspace\fi}
\makeatother

\renewcommand{\lnot}{\mathord{\neg}}

\ifdefined\nequiv

\else
  \def\nequiv{\not\equiv}
\fi

\newcommand{\join}{\vee}
\newcommand{\meet}{\wedge}

\newcommand{\blank}{\mathord{-}}
\newcommand{\pblank}{\mathord{(-)}}

\newcommand{\bcirc}{\bullet}

\newcommand{\embedinto}{\hookrightarrow}
\newcommand{\hoto}{\Rightarrow}

\makeatletter
\newcommand{\profto}{\mathrel{\mathpalette\profto@int\relax}}
\newcommand{\profto@int}[2]{\ooalign{$#1\rightarrow$\cr\hfil$#1\mapsfromchar$\hfil\cr}}
\makeatother

\newcommand{\sharplylt}{\vartriangleleft}

\DeclareMathSymbol{.}{\mathpunct}{letters}{"3A}
\DeclareMathSymbol{:}{\mathrel}{operators}{"3A}

\DeclareMathOperator{\ob}{ob}
\DeclareMathOperator{\mor}{mor}
\DeclareMathOperator{\iso}{iso}

\newcommand{\cotens}{\mathbin{\pitchfork}}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\codom}{codom}

\let\prolim\varprojlim
\let\indlim\varinjlim

\newcommand{\mbfL}{\mathbf{L}}
\newcommand{\mbfU}{\mathbf{U}}
\newcommand{\mbfV}{\mathbf{V}}
\newcommand{\id}{\mathrm{id}}

\AtBeginDocument{\let\emptyset\varnothing}

\newcommand*{\lr}[3]{\mathopen{}\mathclose{\left#1{#2}\right#3}}
\newcommand*{\lmr}[5]{\mathopen{}\mathclose{\left#1{#2}\,\middle#3\,{#4}\right#5}}
\newcommand*{\lrsmash}[3]{\lr#1{\smash{#2}}#3}
\newcommand*{\smashlr}[3]{\mathopen{}\smash{\lr#1{#2}#3}\mathclose{}}
\newcommand*{\ordlr}[3]{\mathord{\left#1{#2}\right#3}}
\newcommand*{\argp}[1]{\ifstrempty{#1}{}{\lr({#1})}}
\newcommand*{\argptwo}[2]{\lr({#1, #2})}
\newcommand*{\argptwotwo}[4]{\lr({#1, #2; #3, #4})}
\newcommand*{\argb}[1]{\ifstrempty{#1}{}{\lr[{#1}]}}
\newcommand*{\parens}[1]{\lr({#1})}
\newcommand*{\ordparens}[1]{\ordlr({#1})}
\newcommand*{\bracket}[1]{\lr[{#1}]}
\newcommand*{\qquote}[1]{\lr\ulcorner{#1}\urcorner}
\newcommand*{\abs}[1]{\ordlr|{#1}|}
\newcommand*{\tuple}[1]{\ordlr({#1})}
\newcommand*{\tuplesmash}[1]{\mathord{\lrsmash({#1})}}
\newcommand*{\prodtuple}[1]{\lr<{#1}>}
\newcommand*{\coprodtuple}[1]{\lr({#1})}

\newcommand*{\setbuilder}[2]{\mathord{\lmr\{{#1}|{#2}\}}}
\newcommand*{\seqbuilder}[2]{\mathord{\lmr({#1}|{#2})}}

\ifdefined\fracslash

\else
  \def\fracslash{\mathbin{/}}
\fi
\ifdefined\divslash

\else
  \def\divslash{\mathbin{/}}
\fi

\newcommand*{\ul}[1]{\smash{\underline{#1}}\vphantom{#1}}

\makeatletter
\newcommand*{\optargp}{\new@ifnextchar\bgroup{\argp}{}}
\newcommand*{\optargptwo}{\new@ifnextchar\bgroup{\expandafter\optargptwo@first}{}}
\newcommand*{\optargptwo@first}[1]{\new@ifnextchar\bgroup{\argptwo{#1}}{\argp{#1}}}
\newcommand*{\optargptwotwo}{\new@ifnextchar\bgroup{\expandafter\optargptwotwo@first}{}}
\newcommand*{\optargptwotwo@first}[2]{\new@ifnextchar\bgroup{\argptwotwo{#1}{#2}}{\argptwo{#1}{#2}}}

\newcommand*{\sbtwo}[2]{\sb{\lr({{#1}, {#2}})}}

\newcommand*{\optsb}{\new@ifnextchar\bgroup{\sb}{}}
\newcommand*{\optsp}{\new@ifnextchar\bgroup{\sp}{}}
\newcommand*{\optsbtwo}{\new@ifnextchar\bgroup{\expandafter\optsbtwo@first}{}}
\newcommand*{\optsbtwo@first}[1]{\new@ifnextchar\bgroup{\sbtwo{#1}}{\sb{#1}}}

\newcommand*{\bracketoptsb}[1][]{\sb{#1}}
\newcommand*{\bracketoptsp}[1][]{\sp{#1}}

\newcommand*{\optsbargp}[1][]{\sb{#1}\optargp}
\newcommand*{\optspargp}[1][]{\sp{#1}\optargp}
\newcommand*{\optsbspargp}[1][]{\sb{#1}\optspargp}
\newcommand*{\optspsbargp}[1][]{\sp{#1}\optsbargp}

\newcommand*{\optsbargptwo}[1][]{\sb{#1}\optargptwo}
\newcommand*{\optspargptwo}[1][]{\sp{#1}\optargptwo}
\newcommand*{\optsbspargptwo}[1][]{\sb{#1}\optspargptwo}
\newcommand*{\optspsbargptwo}[1][]{\sp{#1}\optsbargptwo}

\newcommand*{\set}[1]{\new@ifnextchar\bgroup{\setbuilder{#1}}{\ordlr\{{#1}\}}}
\newcommand*{\seq}[1]{\new@ifnextchar\bgroup{\seqbuilder{#1}}{\tuple{#1}}}
\makeatother

\ifdefined\hash

\else
  \def\hash{\#}
\fi
\newcommand*{\card}[1]{\lr|{#1}|}
\ifdefined\powerset
  \undef\powerset
\else

\fi
\newcommand*{\powerset}[1][]{\mathscr{P}\ifstrempty{#1}{\hairspace}{\sb{#1}} \optargp}
\newcommand*{\setcomp}[1]{{#1}^{\mathsf{c}}}
\newcommand{\rank}{\mathrm{rank}\optargp}
\newcommand{\tcl}{\mathrm{tcl}\optargp}

\newcommand*{\smashsp}[2]{{#1}\sp{\smash{#2}}}

\newcommand*{\subdiv}[1]{\smashsp{#1}{\textrmup{\S}}}

\newcommand*{\op}[1]{\smashsp{#1}{\mathrm{op}}}
\newcommand*{\co}[1]{\smashsp{#1}{\mathrm{co}}}
\newcommand*{\coop}[1]{\smashsp{#1}{\mathrm{co\hairspace op}}}

\newcommand*{\inv}[2][1]{{#2}^{-#1}}

\newcommand*{\succof}[1]{\smashsp{#1}{+}}
\newcommand{\mbfUplus}{\succof{\mbfU}}

\makeatletter
\newcommand*{\ctchoice}[2]{%
  \ifdef{\ct@homstyle}%
  {#2}%
  {#1}}
\newcommand*{\ctchoicetwo}[5]{%
  \ifdef{\ct@homcatstyle}%
  {#2}{%
  \ifdef{\ct@transfstyle}%
  {#3}{%
  \ifdef{\ct@catstyle}%
  {#4}{%
  \ifdef{\ct@homstyle}%
  {#5}{%
  {#1}}}}}}
  
\newcommand*{\DefineCategory}[2]{\DeclareRobustCommand{#1}{\ctchoice{\mathbf{#2}}{\mathbf{#2}}}}
\newcommand*{\DefineBicategory}[2]{\DeclareRobustCommand{#1}{\ctchoicetwo{\mathfrak{#2}}{\mathfrak{#2}}{\mathfrak{#2}}{\mathbf{#2}}{\mathbf{#2}}}}

\newcommand*{\cat}[1]{%
  \begingroup%
  \def\ct@catstyle{cat}%
  #1%
  \endgroup}
\newcommand*{\bicat}[1]{%
  \begingroup
  \def\ct@bicatstyle{bicat}%
  #1%
  \endgroup}
\newcommand*{\Hom}[1][]{%
  \begingroup%
  \def\ct@homstyle{hom}%
  \ifstrempty{#1}{\mathrm{Hom}}{#1}%
  \endgroup%
  \optargptwo}
\newcommand*{\HHom}[1][]{%
  \begingroup%
  \def\ct@homcatstyle{homcat}%
  \ifstrempty{#1}{\mathbf{Hom}}{#1}%
  \endgroup
  \optargptwo}
\newcommand*{\hpty}[1][]{%
  \begingroup%
  \def\ct@transfstyle{transf}%
  \ifstrempty{#1}{\mathrm{Nat}}{#1}%
  \endgroup
  \optargptwotwo}

\makeatother

\DefineCategory{\Set}{Set}
\newcommand{\FinSet}{\ctchoice{\mathbf{FinSet}}{\mathbf{Set}}}
\newcommand{\Setplus}{\ctchoice{\succof{\mathbf{Set}}}{\succof{\mathbf{Set}}}}

\DefineCategory{\CRing}{CRing}

\newcommand{\Cat}{\ctchoicetwo{\mathfrak{Cat}}{\mathbf{Fun}}{\mathbf{Fun}}{\mathbf{Cat}}{\mathrm{Fun}}}

\newcommand*{\commacat}[2]{\ordlr({#1 \mathbin{\downarrow} #2})}

\newcommand*{\slicecat}[2]{\mathord{#1 \mathord{\divslash} #2}}
\newcommand*{\overcat}[2]{\mathord{#1 \sb{\mathord{\divslash} #2}}}
\newcommand*{\undercat}[2]{\mathord{\sp{#1 \mathord{\divslash}} #2}}

\newcommand*{\LKan}[1][]{\mathop{\ifstrempty{#1}{\textrmup{Lan}}{\textrmup{Lan}_{#1}}}}
\newcommand*{\RKan}[1][]{\mathop{\ifstrempty{#1}{\textrmup{Ran}}{\textrmup{Ran}_{#1}}}}

\newcommand{\Kompakt}{\mathbf{K}\optsbspargp}
\newcommand{\Ind}{\mathbf{Ind}\optspsbargp}
\newcommand{\AccFun}{\mathbf{Acc}\optsbspargptwo}

\newcommand{\Nat}{\mathrm{Nat}\argptwo}

\newcommand*{\homs}{\mathpzc{h}\optsb}
\newcommand*{\ophoms}{\mathpzc{h}\optsp}

\newcommand*{\xHom}[3][]{\ifstrempty{#1}{\ordlr[{{#2}, {#3}}]}{\ordlr[{{#2}, {#3}}]\sb{#1}}}
\newcommand*{\ulHom}[1][]{\ifstrempty{#1}{\ul{\Hom}}{\ul{\Hom[#1]}}\optargptwo}

\newcommand*{\Func}[2]{\xHom{#1}{#2}}

\newcommand*{\kwlim}[3][]{\ordlr\lbrace{{#2}, {#3}}\rbrace\sp{#1}}
\newcommand*{\kwcolim}[3][]{{#2} \mathbin{\star\sb{#1}} {#3}}

\usepackage[colorlinks,linkcolor=Blue,citecolor=Blue,urlcolor=blue,pdfpagelabels,pdffitwindow=false]{hyperref}

\usepackage{thmtools}

\declaretheorem[style=plain,parent=section,title=Theorem,refname=theorem,Refname=Theorem]{thm}
\declaretheorem[style=plain,sibling=thm,title=Proposition,refname=proposition,Refname=Proposition]{prop}
\declaretheorem[style=plain,sibling=thm,title=Lemma,refname=lemma,Refname=Lemma]{lem}
\declaretheorem[style=plain,sibling=thm,title=Corollary,refname=corollary,Refname=Corollary]{cor}

\declaretheorem[style=definition,sibling=thm,title=Definition,refname=definition,Refname=Definition]{dfn}

\declaretheorem[style=definition,sibling=thm,title=Example,refname=example,Refname=Example]{example}
\declaretheorem[style=definition,sibling=thm,title=Examples,refname=examples,Refname=Examples]{examples}
\declaretheorem[style=definition,qed=\exercisesymbol,sibling=thm,title=Exercise,refname=exercise,Refname=Exercise]{exercise}

\declaretheoremstyle[style=remark,headfont=\scshape]{remark}
\declaretheorem[style=remark,sibling=thm,title=Remark,refname=remark,Refname=Remark]{remark}

\declaretheorem[style=plain,numbered=no,title=Theorem]{thm*}
\declaretheorem[style=plain,numbered=no,title=Proposition]{prop*}
\declaretheorem[style=remark,numbered=no,title=Remark]{remark*}
\declaretheorem[style=definition,numbered=no,title=Example]{example*}

\def\chapterAutorefname{Chapter}

\makeatletter
\@counteralias{numpar}{thm}
\def\numparAutorefname{Paragraph}
\def\numparautorefname{paragraph}
\newcommand*{\makenumpar}[1][]{%
  \par%
  \refstepcounter{numpar}%
  {\normalfont{\bfseries\textparagraph}\hspace{0.5em}\thenumpar\ifstrempty{#1}{}{ ({\normalfont #1})}.} }
\makeatother

\AtBeginDocument{%
\hyphenation{pull-back pull-backs push-out push-outs co-pro-duct co-pro-ducts co-com-plete sub-ob-ject sub-ob-jects more-over quasi-com-pact de-gen-er-ate pro-vided Gro-then-dieck Law-vere mod-ule sub-al-ge-bra fi-brant co-fi-brant fi-brant-ly co-fi-brant-ly bi-cat-e-go-ry bi-cat-e-gor-ic-al bi-cat-e-gor-ic-al-ly qua-si-cat-e-go-ry qua-si-cat-e-go-ries qua-si-cat-e-go-ric-al}%
}

==> PreludeA.tex <==
\input{Prelude0}

\makeatletter
\renewcommand\footnoterule{%
  \vfill
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}

\renewcommand*{\@makefnmark}{\hbox{\textsuperscript{\normalfont [\LiningNumbers\@thefnmark]}}}
\renewcommand*{\@makefntext}[1]{\parindent 1.0em\noindent\ifdefempty{\@thefnmark}{}{\hb@xt@-1.0em{\hss \normalfont [\LiningNumbers \@thefnmark]}\hspace{1.0em}}#1}
\HyOrg@addtoreset{footnote}{chapter}
\newcommand{\footpar}[1]{\gdef\@thefnmark{}\@footnotetext{#1}}

\newcommand{\hangsecnum}{\def\@seccntformat##1{\llap{\csname the##1\endcsname\quad}}}
\makeatother

\usepackage[natbib,safeinputenc,backend=biber,style=authoryear-comp,bibstyle=authoryear]{biblatex}

\DeclareSortingScheme{mysort}{
  \sort{
    \field{presort}
  }
  \sort[final]{
    \field{sortkey}
  }
  \sort{
    \name{sortname}
    \name{author}
    \name{editor}
    \name{translator}
    \field{sorttitle}
    \field{title}
  }
  \sort{
    \field{sortyear}
    \field{year}
  }
  \sort{
    \field{month}
  }
  \sort{
    \field{day}
  }
  \sort{
    \field{journal}
  }
  \sort{
    \field[padside=left,padwidth=4,padchar=0]{volume}
    \literal{0000}
  }
  \sort{
    \field{series}
  }
  \sort{
    \field[padside=left,padwidth=4,padchar=0]{number}
    \literal{0000}
  }
  \sort{
    \field{sorttitle}
    \field{title}
  }
}

\ExecuteBibliographyOptions{sorting=mysort,block=space,useprefix=true,maxcitenames=3,maxbibnames=10,mergedate=false,pagetracker=false}

%%% BEGIN BibLaTeX style

\setlength{\bibnamesep}{\baselineskip}
\renewcommand*{\bibnamedash}{}
\newcommand*{\authoryearpunct}{\hspace*{-\bibhang}\bibsentence}
\renewcommand*{\labelnamepunct}{\addspace}

\makeatletter

\appto\citesetup{\LiningNumbers}

\renewbibmacro*{cite:label}{%
  \iffieldundef{label}
    {\printtext[bibhyperref]{\printfield[citetitle]{labeltitle}}}
    {\printtext[bibhyperref]{\printfield{label}}}}

\renewbibmacro*{date+extrayear}{%
  \iffieldundef{shorthand}
    {\iffieldundef{labelyear}
      {}
      {\printtext[brackets]{\printfield{labelyear}\printfield{extrayear}}}\addspace}
    {\printtext[brackets]{\printfield{shorthand}}}}

\renewbibmacro*{author}{%
  \ifboolexpr{
    test \ifuseauthor
    and
    not test {\ifnameundef{author}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\usebibmacro{bbx:savehash}%
        \printnames{author}%
    \newline\setunit{\authoryearpunct}}%
     \iffieldundef{authortype}
       {}
       {\usebibmacro{authorstrg}%
    \setunit{\addspace}}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\renewbibmacro*{bbx:editor}[1]{%
  \ifboolexpr{
    test \ifuseeditor
    and
    not test {\ifnameundef{editor}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\printnames{editor}%
    \newline\setunit{\authoryearpunct}%
    \usebibmacro{bbx:savehash}}%
     \usebibmacro{#1}%
     \clearname{editor}%
     \setunit{\addspace}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\renewbibmacro*{bbx:translator}[1]{%
  \ifboolexpr{
    test \ifusetranslator
    and
    not test {\ifnameundef{translator}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\printnames{translator}%
    \newline\setunit{\authoryearpunct}%
    \usebibmacro{bbx:savehash}}%
     \usebibmacro{translator+othersstrg}%
     \clearname{translator}%
     \setunit{\addspace}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\makeatother

%%% END BibLaTeX style

\renewcommand*{\mkbibparens}[1]{{\ifcitation{\bibleftbracket#1\bibrightbracket}%
    {\bibleftparen#1\bibrightparen}}}
\renewcommand*{\bibopenparen}[1]{{\ifcitation{\bibleftbracket#1}{\bibleftparen#1}}}
\renewcommand*{\bibcloseparen}{{\ifcitation{\bibrightbracket}{\bibrightparen}}}
\appto\bibsetup{\raggedright}
\appto\bibfont{\LiningNumbers\small}

\addbibresource{Bibliography.bib}

